The Parameterised Complexity of Temporal Motif Counting, and a Lov\'asz-Style Isomorphism Theorem

We study the structural expressivity and the parameterised complexity of counting homomorphisms from small temporal patterns to large temporal graphs. Here, a temporal pattern $P$ consists of a graph together with a partial order on its edges, and a homomorphism from $P$ to a temporal graph must not only preserve edges, but also satisfy the temporal constraints imposed by the partial order of the edge set of the pattern. The main results of this work are three-fold: First, we prove a temporal Lov\'asz-style theorem, stating that two temporal graphs are isomorphic (under a natural definition of temporal isomorphisms) if and only if they have the same number of homomorphisms from all temporal patterns. Second, we introduce a cliquewidth-based measure on temporal patterns, called the temporally order-augmented dual width, the "toadwidth" for short, and show that counting temporal homomorphisms is fixed-parameter tractable for temporal patterns of bounded toadwidth. Third, we provide a parameterised complexity dichotomy with an explicit tractability criterion for counting homomorphisms from totally ordered temporal patterns, classified along their underlying graph structure.

==> fig-label-classes.tex <==
\begin{tikzpicture}[scale=0.65, every node/.style={circle, draw, minimum size=2.5mm}, every edge quotes/.style = {auto, font=\footnotesize, sloped}]

%%%Top layeer - Primal graph

%%First oval
\draw (0,10.5) ellipse (1.3cm and 4cm);

\node[fill=gray!30] (ue) at (-0.7, 10.5) {};
\node[fill=gray!30] (ve) at (0.7, 10.5) {};
\draw[thick] (ue) to (ve);

%%Second oval
\draw (4,10.5) ellipse (1.3cm and 4cm);

\node[fill=gray!30] (ue1) at (3.3, 11.5) {};
\node[fill=gray!30] (ve1) at (4.7, 11.5) {};
\draw[thick] (ue1) to (ve1);

\node[fill=gray!30] (ue2) at (3.3, 9.5) {};
\node[fill=gray!30] (ve2) at (4.7, 9.5) {};
\draw[thick] (ue2) to (ve2);

%%Third oval
\draw (8,10.5) ellipse (1.3cm and 4cm);

\node[fill=gray!30] (ue3) at (7.3, 10.5) {};
\node[fill=gray!30] (ve3) at (8.7, 11.5) {};
\node[fill=gray!30] (ve4) at (8.7, 9.5) {};
\draw[thick] (ue3) to (ve3);
\draw[thick] (ue3) to (ve4);

%%Fourth oval
\draw (12,10.5) ellipse (1.3cm and 4cm);

\node[fill=gray!30] (ue5) at (11.3, 10.5) {};
\node[fill=gray!30] (ve5) at (12.7, 12.0) {};
\node[fill=gray!30] (ve6) at (12.7, 10.5) {};
\node[fill=gray!30] (ve7) at (12.7, 9.0) {};
\draw[thick] (ue5) to (ve5);
\draw[thick] (ue5) to (ve6);
\draw[thick] (ue5) to (ve7);


%%Fifth oval
\draw (16.5,10.5) ellipse (1.5cm and 4cm);

\node[fill=gray!30] (ue8) at (15.8, 12.0) {};
\node[fill=gray!30] (ve8) at (17.2, 13.0) {};
\node[fill=gray!30] (ve9) at (17.2, 11.0) {};
\draw[thick] (ue8) to (ve8);
\draw[thick] (ue8) to (ve9);

\node[fill=gray!30] (ue10) at (15.8, 9.0) {};
\node[fill=gray!30] (ve10) at (17.2, 9.0) {};
\draw[thick] (ue10) to (ve10);


%%Sixth oval
\draw (21,10.5) ellipse (1.5cm and 4cm);

\node[fill=gray!30] (ue11) at (20.3, 12) {};
\node[fill=gray!30] (ve11) at (21.7, 13.0) {};
\node[fill=gray!30] (ve12) at (21.7, 12.0) {};
\node[fill=gray!30] (ve13) at (21.7, 11) {};
\draw[thick] (ue11) to (ve11);
\draw[thick] (ue11) to (ve12);
\draw[thick] (ue11) to (ve13);

\node[fill=gray!30] (ue14) at (20.3, 9) {};
\node[fill=gray!30] (ve14) at (21.7, 9.6) {};
\node[fill=gray!30] (ve15) at (21.7, 8.4) {};
\draw[thick] (ue14) to (ve14);
\draw[thick] (ue14) to (ve15);


%%%Bottom layeer - Line graph

\draw (0,1.5) ellipse (1.3cm and 4cm);

\node[fill=gray!30] (e) at (0, 1.5) {$e$};


\draw (4,1.5) ellipse (1.3cm and 4cm);

\node[fill=gray!30] (e1) at (4, 2.5) {$e_1$};
\node[fill=gray!30] (e2) at (4, 0.5) {$e_2$};


\draw (8,1.5) ellipse (1.3cm and 4cm);

\node[fill=gray!30] (e3) at (8, 2.5) {$e_3$};
\node[fill=gray!30] (e4) at (8, 0.5) {$e_4$};
\draw[thick] (e3) to (e4);


\draw (12,1.5) ellipse (1.6cm and 4cm);

\node[fill=gray!30] (e5) at (12, 2.2) {$e_5$};
\node[fill=gray!30] (e6) at (11, 0.8) {$e_6$};
\node[fill=gray!30] (e7) at (13, 0.8) {$e_7$};
\draw[thick] (e5) to (e6);
\draw[thick] (e6) to (e7);
\draw[thick] (e5) to (e7);


\draw (16.5,1.5) ellipse (1.6cm and 4cm);

\node[fill=gray!30] (e8) at (16.5, 3.2) {$e_8$};
\node[fill=gray!30] (e9) at (16.5, 1.5) {$e_9$};
\draw[thick] (e8) to (e9);

\node[fill=gray!30] (e10) at (16.5, -0.5) {$e_{10}$};



\draw (21,1.5) ellipse (1.8cm and 4cm);

\node[fill=gray!30] (e11) at (21, 4.2) {$e_{11}$};
\node[fill=gray!30] (e12) at (20, 2.8) {$e_{12}$};
\node[fill=gray!30] (e13) at (22, 2.8) {$e_{13}$};
\draw[thick] (e11) to (e12);
\draw[thick] (e11) to (e13);
\draw[thick] (e12) to (e13);

\node[fill=gray!30] (e14) at (21, 0.4) {$e_{14}$};
\node[fill=gray!30] (e15) at (21, -1.4) {$e_{15}$};
\draw[thick] (e14) to (e15);



\begin{comment}
% Vertices
\node[fill=gray!30] (a) at (0, 1.5) {$\hat{a}$};
\node (v1) at (2, 2.5) {$v_1$};
\node (v2) at (2, 0.5) {$v_2$};

% Multi-edges from \hat{a} to v1
\draw[thick] (a) to[bend left=20] (v1);
\draw[thick] (a) to[bend right=20] (v1);

% Multi-edges from \hat{a} to v2
\draw[thick] (a) to[bend left=20] (v2);
\draw[thick] (a) to[bend right=20] (v2);
\end{comment}
\end{tikzpicture}



==> fig-viable.tex <==

\begin{tikzpicture}[scale=0.5, every node/.style={circle, minimum size=2.5mm}, every edge quotes/.style = {auto, font=\footnotesize, sloped}]


%%star
\node[minimum size=6mm, draw,fill=gray!30] (u) at (0.0, 9.0) {};
\node[draw, fill=gray!30] (x1) at (2.0, 11.0) {};
\node[draw, fill=gray!30] (x2) at (2.0, 10.0) {};
\node[draw, fill=gray!30] (x3) at (2.0, 9.0) {};
\node[draw, fill=gray!30] (x4) at (2.0, 8.0) {};
\node[draw, fill=gray!30] (x5) at (2.0, 7.0) {};

\draw[thick] (u) to (x5);
\draw[thick] (u) to (x4);
\draw[thick] (u) to (x3);
\draw[thick] (u) to (x2);
\draw[thick] (u) to (x1);

\node[] (H1) at (1.0, 5.7) {$H_1$};

%%union of two disjoint stars -- one is an edge
\node[minimum size=6mm, draw, fill=gray!30] (u) at (5.0, 10.0) {};
\node[draw, fill=gray!30] (x1) at (7.0, 11.5) {};
\node[draw, fill=gray!30] (x2) at (7.0, 10.5) {};
\node[draw, fill=gray!30] (x3) at (7.0, 9.5) {};
\node[draw, fill=gray!30] (x4) at (7.0, 8.5) {};



\draw[thick] (u) to (x4);
\draw[thick] (u) to (x3);
\draw[thick] (u) to (x2);
\draw[thick] (u) to (x1);

\node[minimum size=6mm, draw, fill=gray!30] (v) at (5.0, 7.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (y1) at (7.0, 7.0) {};

\draw[thick] (v) to (y1);

\node[] (H2) at (6.0, 5.7) {$H_2$};

%%%union of two disjoint stars 
\node[minimum size=6mm, draw, fill=gray!30] (u) at (10.0, 11.0) {};
\node[draw, fill=gray!30] (x1) at (12.0, 12.0) {};
\node[draw, fill=gray!30] (x2) at (12.0, 11.0) {};
\node[draw, fill=gray!30] (x3) at (12.0, 10.0) {};

\draw[thick] (u) to (x3);
\draw[thick] (u) to (x2);
\draw[thick] (u) to (x1);

\node[minimum size=6mm, draw, fill=gray!30] (v) at (10.0, 7.5) {};
\node[draw, fill=gray!30] (y1) at (12.0, 8.5) {};
\node[draw, fill=gray!30] (y2) at (12.0, 7.5) {};
\node[draw, fill=gray!30] (y3) at (12.0, 6.5) {};

\draw[thick] (v) to (y3);
\draw[thick] (v) to (y2);
\draw[thick] (v) to (y1);

\node[] (H3) at (11.0, 5.7) {$H_3$};

%%%two stars with paths -- both stars are single vertices

\node[minimum size=6mm, draw, fill=gray!30] (u) at (16.0, 11.0) {};

\node[draw, fill=gray!0] (p1) at (15.0, 9.0) {};
\node[draw, fill=gray!0] (p2) at (16.0, 9.0) {};
\node[draw, fill=gray!0] (p3) at (17.0, 9.0) {};

\node[minimum size=6mm, draw, fill=gray!30] (v) at (16.0, 7.0) {};

\draw[thick] (u) to (p1);
\draw[thick] (u) to (p2);
\draw[thick] (u) to (p3);

\draw[thick] (v) to (p1);
\draw[thick] (v) to (p2);
\draw[thick] (v) to (p3);

\node[] (H4) at (16.0, 5.7) {$H_4$};

%%%two stars with paths -- one is a single edge and the other is a  single vertex

\node[minimum size=6mm, draw, fill=gray!30] (u1) at (20.5, 13.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (u2) at (20.5, 11.0) {};

\node[draw, fill=gray!0] (p1) at (20.0, 9.0) {};
\node[draw, fill=gray!0] (p2) at (21.0, 9.0) {};


\node[minimum size=6mm, draw, fill=gray!30] (v) at (20.5, 7.0) {};

\draw[thick] (u1) to (u2);
\draw[thick] (u2) to (p1);
\draw[thick] (u2) to (p2);
\draw[thick] (v) to (p1);
\draw[thick] (v) to (p2);

\node[] (H5) at (20.5, 5.7) {$H_5$};

%%%two stars with paths -- one is a single vertex

\node[draw, fill=gray!30] (x1) at (24.0, 13.0) {};
\node[draw, fill=gray!30] (x2) at (25.0, 13.0) {};
\node[draw, fill=gray!30] (x3) at (26.0, 13.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (u) at (25.0, 11.0) {};

\node[draw, fill=gray!0] (p1) at (25.0, 9.0) {};



\node[minimum size=6mm, draw, fill=gray!30] (v) at (25.0, 7.0) {};

\draw[thick] (u) to (x1);
\draw[thick] (u) to (x2);
\draw[thick] (u) to (x3);
\draw[thick] (u) to (p1);
\draw[thick] (v) to (p1);

\node[] (H6) at (25.0, 5.7) {$H_6$};


%%%two stars with paths -- both stars are single edges

\node[minimum size=6mm, draw, fill=gray!30] (u1) at (-2.0, 3.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (u2) at (0.0, 3.0) {};

\node[draw, fill=gray!0] (p1) at (2.0, 3.5) {};
\node[draw, fill=gray!0] (p2) at (2.0, 2.5) {};

\node[minimum size=6mm, draw, fill=gray!30] (v1) at (4.0, 3.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (v2) at (6.0, 3.0) {};

\draw[thick] (u1) to (u2);
\draw[thick] (u2) to (p1);
\draw[thick] (u2) to (p2);
\draw[thick] (v1) to (p1);
\draw[thick] (v1) to (p2);
\draw[thick] (v1) to (v2);

\node[] (H7) at (2.0, 1.5) {$H_7$};

%%%two stars with a path -- one star is a single edge

\node[minimum size=6mm, draw, fill=gray!30] (u) at (11.0, 3.0) {};
\node[draw, fill=gray!30] (x1) at (9.0, 3.5) {};
\node[draw, fill=gray!30] (x2) at (9.0, 2.5) {};


\node[draw, fill=gray!0] (p1) at (13.0, 3.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (v1) at (15.0, 3.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (v2) at (17.0, 3.0) {};


\draw[thick] (u) to (x2);
\draw[thick] (u) to (x1);

\draw[thick] (u) to (p1);
\draw[thick] (v1) to (p1);
\draw[thick] (v1) to (v2);

\node[] (H8) at (13.0, 1.5) {$H_8$};

%%%two stars with a path 

\node[minimum size=6mm, draw, fill=gray!30] (u) at (22.0, 3.0) {};
\node[draw, fill=gray!30] (x1) at (20.0, 3.5) {};
\node[draw, fill=gray!30] (x2) at (20.0, 2.5) {};


\node[draw, fill=gray!0] (p1) at (24.0, 3.0) {};
\node[minimum size=6mm, draw, fill=gray!30] (v) at (26.0, 3.0) {};
\node[draw, fill=gray!30] (y1) at (28.0, 4.0) {};
\node[draw, fill=gray!30] (y2) at (28.0, 3.0) {};
\node[draw, fill=gray!30] (y3) at (28.0, 2.0) {};

\draw[thick] (u) to (x2);
\draw[thick] (u) to (x1);

\draw[thick] (u) to (p1);
\draw[thick] (v) to (p1);

\draw[thick] (v) to (y1);
\draw[thick] (v) to (y2);
\draw[thick] (v) to (y3);
\node[] (H9) at (24.0, 1.5) {$H_9$};
\end{tikzpicture}


==> tikzlibraryconference.code.tex <==
%\documentclass{standalone}
%\usepackage{tikz}

\usepackage{ifthen}
\usetikzlibrary{calc,shapes,fit}
\usetikzlibrary{decorations.markings}


\tikzset{vertex/.style={circle, fill, inner sep=1pt, outer sep=1.3pt}}
\tikzset{svertex/.style={circle,draw=white, line width=1.2pt,fill=black, inner sep=1.8pt, outer sep=0pt}}
\tikzset{ssvertex/.style={circle,fill=black, inner sep=.7pt, outer sep=-.75pt}}
\tikzset{sssvertex/.style={circle,fill=black, inner sep=.5pt, outer sep=-.6pt}}
\tikzset{bbvertex/.style={circle,fill=black, inner sep=.8pt, outer sep=-.9pt}}
\tikzset{bag/.style={gray,minimum size=20pt,diamond,draw,rounded corners=4pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}
\tikzset{sbag/.style={gray,minimum size=15pt,diamond,draw,rounded corners=2pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}

%\tikzset{hom/.style={black}}
%\tikzset{shom/.style={white,double=black, thick}}

\def\ccol{red}
\def\ecol{blue}
\def\icol{red!50!blue}

\tikzset{ssedge/.style={white,thick, double=black, double distance=2pt}}
\tikzset{tedge/.style={white,thick, double=black, double distance=1pt}}
\tikzset{sssedge/.style={white,thick, double=black, double distance=1.5pt}}
\tikzset{stedge/.style={white,thin, double=gray, double distance=.6pt}}
\tikzset{sstedge/.style={white,thin, double=gray!60, double distance=.6pt}}
\tikzset{dedge/.style={gray,thick, double=white, double distance=9pt}}
\tikzset{sdedge/.style={gray,thick, double=white, double distance=5pt}}

\tikzset{sty/.store in=\sty,sty=10}

\tikzset{cross/.style={cross out, draw, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer         sep=0pt}}

\tikzset{tvertex/.style={circle, fill, inner sep=1pt, outer sep=1.3pt}}
\tikzset{btvertex/.style={draw,circle,dashed,very thin,gray,inner sep=4pt, outer sep=-1pt}}
\tikzset{bbtvertex/.style={draw,dashed,thin,gray,inner sep=5.5pt, outer sep=-.5pt}}

\def\dotedge[#1](#2)--(#3);{%
    \draw[#1,dotted] ($(#2)!.33!(#3)$) -- ($(#2)!.66!(#3)$);%
    \draw[#1] ($(#2)!.64!(#3)$) -- (#3);%
    \draw[#1] (#2) -- ($(#2)!.35!(#3)$);%
}

%% slice from pgfpie

% #8:#1 center
% #7:#2 radius
% #1:#3 begin angle
% #2:#4 end angle
% #5:#5 explode
% #6: fill color

% #3: number
% #4: label
% #6: fill color

\makeatletter
\tikzset{slsty/.store in=\@sty,slsty=}
\def\slice#1#2#3#4#5#6#7{
    \pgfmathsetmacro{\midangle}{0.5*(#3)+0.5*(#4)}
    \pgfmathsetmacro{\sliceradius}{#2+#5}
    \path (#1) -- ++(\midangle:#5) coordinate(O);
    \node[inner sep=1pt, outer sep=1.2pt] (#7) at (O) {};
    \draw[line join=round, color=#6, fill=#6, \@sty] (O) -- ++(#3:#2) arc (#3:#4:#2) -- cycle;
}

% #1 coordinate
% #2 split
% #3 coordinate name
\def\kowaen#1#2#3;{
    \foreach \i/\j/\k [count=\c from 1] in {#2} {
        \slice{#1}{1.3pt}{\i}{\j}{2pt}{\k}{#3-\c};
    }
}

\def\coledge(#1|#2)--(#3|#4);{
    \draw[tedge] (#1) -- (#3);
    \draw[tedge, double=#2] (#1) -- ($(#1)!.35!(#3)$);
    \draw[tedge, double=#4] (#3) -- ($(#3)!.35!(#1)$);
}

\tikzset{
    every label/.append style={font=\tiny, label distance=-3}
}

\tikzset{
    pics/torus/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }
            \pgfmathsetmacro{\n}{int(#1-1)}

            \foreach\j in {1,...,#1} {
                \pgfmathsetmacro{\xodd}{isodd(\j) && \j > 1 && \j <= \n}
                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 1 && \j <= \n}
                \ifthenelse{\xodd=1}{
                    \node[rotate=8,regular polygon,regular polygon sides=#1,minimum
                    size=\j*35pt] (p\j) {};
                    }{
                    \ifthenelse{\xeven=1}{
                        \draw[\es,double=black!20] circle (\j*17.6pt);
                        \node[rotate=-10/\j,regular polygon,regular polygon sides=#1,minimum
                        size=\j*35pt] (p\j) {};
                        }{
                        \node[regular polygon,regular polygon sides=#1,minimum
                        size=\j*35pt] (p\j) {};
                    }
                }

                \foreach\l in {1,...,#1}{
                    \pgfmathsetmacro{\de}{(9 * \l + 7.4) * 40 / #1}
                    \pgfmathsetmacro{\dee}{(9 * \l + 6) * 40 / #1}
                    \draw[very thick,white] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    \draw[thick,dotted,black!20] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    \node[inner sep=1.8pt, circle,fill= white] (\j\l) at (p\j.corner \l) {};
                    \ifthenelse{\xeven=1}{
                        \node[\vs,black!20] (\j\l) at (p\j.corner \l) {};
                    }{}
                }
            }
            \foreach\j in {1,...,#1} {
                \foreach\l in {1,...,#1}{

                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 2}
                \pgfmathsetmacro{\xodd}{isodd(\j) && \j > 2}
                \pgfmathsetmacro{\jmt}{int(\j - 2)}
                \ifthenelse{\xeven=1}{
                    \dotedge[\es,double=black!20](\j\l)--(\jmt\l);
                }{}
                \ifthenelse{\xodd=1}{
                    \dotedge[\es,double=black](\j\l)--(\jmt\l);
                }{}
            }
            \dotedge[\es,double=black!20](#1\j)--(\n\j);
            \dotedge[\es,double=black!20](1\j)--(2\j);
        }
        \foreach\j in {1,...,#1} {
                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 1 && \j <= \n}
                \ifthenelse{\xeven=1}{}{
                    \draw[\es] circle (\j*17.6pt);
                    \foreach\l in {1,...,#1}{
                        \node[inner sep=1.8pt, circle,fill= white] (\j\l) at (p\j.corner \l) {};
                        \node[\vs] (\j\l) at (p\j.corner \l) {};
                        \ifthenelse{\j=1}{
                            \pgfmathsetmacro{\de}{(9 * \l + 9) * 40 / #1}
                            \pgfmathsetmacro{\dee}{(9 * \l + 4.5) * 40 / #1}
                            }{
                            \pgfmathsetmacro{\de}{(9 * \l + 7.5) * 40 / #1}
                            \pgfmathsetmacro{\dee}{(9 * \l + 6.1) * 40 / #1}
                        }
                        \draw[very thick,white] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                        \draw[thick,dotted] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    }
                }
            }
        }
    }
}
\tikzset{
    pics/grid/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }
            \pgfmathsetmacro{\n}{int(#1-1)}
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\xedgee=1}{
                        \draw[smooth,\ess]
                        (\j\l.east)
                        to ($(\j\l.east) + (.35, 0)$)
                        to[out=0, in=0] ($(\j\l.east) + (.35, -0.25)$)
                        to ($(1\l.west) - (.15, 0.25)$)
                        to[out=180,in=180] ($(1\l.west) - (.15, 0)$)
                        to (1\l.west)
                        ;
                    }{}
                    }{
                    \node[inner sep=1.3ex] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yodd=1}{
                        \draw[dotted,\es] (\j\l.west) -- (\j\l.east);
                        }{
                        \ifthenelse{\xodd=1}{
                            \draw[dotted,\es] (\j\l.north) -- (\j\l.south);
                            }{
                }}}
            }
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yedgee=1}{
                        \draw[smooth,\ess]
                        (\j\l.north)
                        to ($(\j\l.north) + (0,.15)$)
                        to[out=90, in=90] ($(\j\l.north) + (.25, 0.15)$)
                        to ($(\j1.south) - (-.25, 0.35)$)
                        to[out=270,in=270] ($(\j1.south) - (0,.35)$)
                        to (\j1.south)
                        ;
                    }{}
                    }{
                    \node[inner sep=1.3ex] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yodd=1}{
                        \draw[dotted,\es] (\j\l.west) -- (\j\l.east);
                        }{
                        \ifthenelse{\xodd=1}{
                            \draw[dotted,\es] (\j\l.north) -- (\j\l.south);
                            }{
                }}}
            }
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}}
                {\ifthenelse{\edge=1}{\def\tp{edge}}
                {\def\tp{inner}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\normalgrid=1}{
                        \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                        }{
                        \ifthenelse{\mode=0}{
                            \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.065)$) {};
                            \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.065,0)$) {};
                            \node[ssvertex] (s\j\l) at ($(\j\l.south)+(0,.065)$) {};
                            \node[ssvertex] (w\j\l) at ($(\j\l.west)+(.065,0)$) {};

                            % \draw[ssedge] (n\j\l) -- (s\j\l);
                            % \draw[ssedge] (s\j\l) -- (e\j\l);
                            }{
                            \node[sssvertex] (ne\j\l) at ($(\j\l.north east)+(-0.05,-.05)$) {};
                            \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.06)$) {};
                            \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.06,0)$) {};
                            \node[ssvertex] (s\j\l) at ($(\j\l.south)+(0,.06)$) {};
                            \node[ssvertex] (w\j\l) at ($(\j\l.west)+(.06,0)$) {};
                            \node[bbvertex] (sw\j\l) at ($(\j\l.south west)-(-0.05,-.05)$) {};

                            \ifthenelse{#2=15}{
                                \draw[tedge] (ne\j\l) -- (sw\j\l);
                                \draw[sssedge] (w\j\l) -- (n\j\l) -- (e\j\l) -- (s\j\l);
                            }{}
                            \ifthenelse{#2=16}{
                                \draw[tedge] (w\j\l) -- (ne\j\l);
                                \draw[sssedge] (n\j\l) -- (s\j\l);
                                \draw[tedge] (ne\j\l) -- (e\j\l) -- (sw\j\l) -- (w\j\l);
                                \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.06)$) {};
                            }{}
                            \ifthenelse{#2=17}{
                                \draw[tedge] (s\j\l) -- (ne\j\l);
                                \draw[sssedge] (w\j\l) -- (e\j\l);
                                \draw[tedge] (sw\j\l) -- (n\j\l) -- (ne\j\l)  (s\j\l) -- (sw\j\l);
                                \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.06,0)$) {};
                            }{}
                        }
                        \ifthenelse{#2=1}{\draw[ssedge] (n\j\l) -- (s\j\l);}{}
                        \ifthenelse{#2=2}{\draw[ssedge] (w\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=3}{\draw[ssedge] (n\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=4}{\draw[ssedge] (s\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=5}{\draw[ssedge] (n\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=6}{\draw[ssedge] (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=7}{\draw[ssedge] (n\j\l) -- (e\j\l);
                        \draw[ssedge] (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=8}{\draw[ssedge] (s\j\l) -- (e\j\l);
                        \draw[ssedge] (n\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=9}{
                            \draw[ssedge] (e\j\l) -- (w\j\l);
                            \draw[ssedge] (s\j\l) -- (n\j\l);
                        }{}
                        \ifthenelse{#2=10}{\draw[ssedge] (n\j\l) -- (e\j\l) -- (s\j\l);}{}
                        \ifthenelse{#2=11}{\draw[ssedge] (e\j\l) -- (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=12}{\draw[ssedge] (s\j\l) -- (w\j\l) -- (n\j\l);}{}
                        \ifthenelse{#2=13}{\draw[ssedge] (w\j\l) -- (n\j\l) -- (e\j\l);}{}

                    }
                    \ifthenelse{\j>1}{
                        \pgfmathsetmacro{\up}{int(\j-1)}
                        \pgfmathsetmacro{\upp}{int(\j-2)}
                        \draw[\es] (\up\l) -- (\j\l);
                        \draw[\es] (\upp\l) -- (\up\l);
                    }{}
                    \ifthenelse{\l>1}{
                        \pgfmathsetmacro{\left}{int(\l-1)}
                        \pgfmathsetmacro{\leftt}{int(\l-2)}
                        \draw[\es] (\j\left) -- (\j\l);
                        \draw[\es] (\j\left) -- (\j\leftt);
                    }{}

                }{}
            }
        }
    }
}

\tikzset{
    pics/gridgrid/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}
            \begin{scope}[opacity=0.4]
                \begin{scope}[opacity=0.2]
                    \pic[sty=\bg1] (2) at (2, 2) {grid=#1/#2};
                \end{scope}
                \pic[sty=\bg1] (1) at (1, 1) {grid=#1/#2};
            \end{scope}
            \pic[sty=\bg1] (0) at (0, 0) {grid=#1/#2};

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \pgfmathsetmacro{\n}{int(#1-1)}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }

            \definecolor{l2b}{rgb}{.6,.6,.6}
            \definecolor{l1b}{rgb}{.8,.8,.8}
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}}
                {\ifthenelse{\edge=1}{\def\tp{edge}}
                {\def\tp{inner}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\normalgrid=1}
                    {

                        \draw[\es,double=black!60,dotted]  ($(0\j\l)!0.35!(1\j\l)$) --
                        ($(0\j\l)!0.64!(1\j\l)$);
                        \draw[\es,double=black!30,dotted]  ($(1\j\l)!0.35!(2\j\l)$) --
                        ($(1\j\l)!0.64!(2\j\l)$);
                        \draw[\es,double=black] (0\j\l) -- ($(0\j\l)!0.37!(1\j\l)$);
                        \draw[\es,double=black!40] (1\j\l) -- ($(0\j\l)!0.62!(1\j\l)$);

                        \draw[\es,double=black!40] (1\j\l) -- ($(1\j\l)!0.37!(2\j\l)$);
                        \draw[\es,double=black!20] (2\j\l) -- ($(1\j\l)!0.62!(2\j\l)$);
                        \draw[smooth,\ess]
                        (2\j\l.north east)
                        to ($(2\j\l.north east) + (.15,.15)$)
                        to[out=45, in=45] ($(2\j\l.north east) + (.45, 0.15)$)
                        to ($(0\j\l.south west) - (-0.05, 0.25)$)
                        to[out=270-45,in=270-45] ($(0\j\l.south west) - (.25,.25)$)
                        to (0\j\l.south west)
                        ;
                        }{
                        \draw[\es,double=black!60,dotted]  ($(0\j\l)!0.35!(1\j\l)$) --
                        ($(0\j\l)!0.64!(1\j\l)$);
                        \draw[\es,double=black!30,dotted]  ($(1\j\l)!0.35!(2\j\l)$) --
                        ($(1\j\l)!0.64!(2\j\l)$);
                        \draw[\es,double=black] (0\j\l) -- ($(0\j\l)!0.37!(1\j\l)$);
                        \draw[\es,double=black!40] (1\j\l) -- ($(0\j\l)!0.62!(1\j\l)$);

                        \draw[\es,double=black!40] (1\j\l) -- ($(1\j\l)!0.37!(2\j\l)$);
                        \draw[\es,double=black!20] (2\j\l) -- ($(1\j\l)!0.62!(2\j\l)$);
                        \draw[smooth,sstedge]
                        ($(2\j\l.north east) - (.02,.02)$)
                        to ($(2\j\l.north east) + (.05,.05)$)
                        to[out=45, in=45] ($(2\j\l.north east) + (.35, 0.05)$)
                        to ($(0\j\l.south west) - (-0.15, 0.15)$)
                        to[out=270-45,in=270-45] ($(0\j\l.south west) - (.15,.15)$)
                        to (0\j\l.south west)
                        ;

                    }
                }{}
            }

        }
    }
}


\makeatother

